Understanding Fashion Cycles as a Social Choice

We present a formal model for studying fashion trends, in terms of three parameters of fashionable items: (1) their innate utility; (2) individual boredom associated with repeated usage of an item; and (3) social influences associated with the preferences from other people. While there are several works that emphasize the effect of social influence in understanding fashion trends, in this paper we show how boredom plays a strong role in both individual and social choices. We show how boredom can be used to explain the cyclic choices in several scenarios such as an individual who has to pick a restaurant to visit every day, or a society that has to repeatedly `vote' on a single fashion style from a collection. We formally show that a society that votes for a single fashion style can be viewed as a single individual cycling through different choices. In our model, the utility of an item gets discounted by the amount of boredom that has accumulated over the past; this boredom increases with every use of the item and decays exponentially when not used. We address the problem of optimally choosing items for usage, so as to maximize over-all satisfaction, i.e., composite utility, over a period of time. First we show that the simple greedy heuristic of always choosing the item with the maximum current composite utility can be arbitrarily worse than the optimal. Second, we prove that even with just a single individual, determining the optimal strategy for choosing items is NP-hard. Third, we show that a simple modification to the greedy algorithm that simply doubles the boredom of each item is a provably close approximation to the optimal strategy. Finally, we present an experimental study over real-world data collected from query logs to compare our algorithms.

==> influence.tex <==
\section{Effect of Influence}
Let us now understand the effect of influence on utilities. We will temporarily
ignore the effect of boredom and assume that there is a social network and peoples

Our utility depends not only on our evaluation but also on the utility
of others. The valuation diffuses through the social network as
described.

Think of only one item. let $u_j$ denote the utility to person $j$. 
So $u = (u_1,...,u_n)$ is the vector of utilities for an item that is a function of time, then
the utility for the first person at time $t+1$ is given by,

$u_1(t+1) = w_{1,1} u_1(t) + w_{1,2} u_2(t) +.. + w_{1,n} u_n(t)$.
 
This gives the recurrence $u(t+1)  = W u(t)$, where $W$ is the weight influence matrix.
If all weights are positive then there is a fixed point given by, 
$u = e^t e u(0)$ where $e$ is the top eigen vector.

Thus the total welfare by introducing fashion $i$ is given by $\sum u_j(t) = c^t u(0)$ for some fixed vector $c$ that 
depends on the influence matrix $W$.
One can view $c$ is the social influence vector. $c_j$ is the amount by which he utility
$u_j$ affects the welfare of society.

\begin{theorem}
If all influences are positive then, ignoring the effect of boredom, in equilibrium the welfare of a society from a particular 
item is simply a weighted linear combination of the utilties of the different individuals
\end{theorem}


==> marketsegments.tex <==
\section{Multiple Market Segments}

Chains of Influence:
[Fashion Conscious Segment]->[Followers]

Consider a case when the market consists of two segments, one fashion
conscious segment and another segment that imitates the previous
segment. There may be a delay between the introduction of a fashion to
the first segment to the point where it spreads to the rest of
society. In such a case the first segment drives the fashion choices
based on its combined utility and boredom coefficients and these
choices are propagated to the remaning segment. Thus fashion is
essentially the boredom countering choices made by the influential set
of people in the society.

Negative influence:

[Fashion Conscious Segment]->[Followers]- -ve -> first segment.


==> newproofs.tex <==
\section{Technical details}
\label{sec:proofs}

\subsection{Individual choice}

The following lemma is used in the proof of Theorem~\ref{thm:gap1}.

\begin{lemma}\label{lem:mem}
$\sum_i M_i(t)\leq 1$, and $\sum_i M_i(t) \to 1$ for large $t$. When $t=\Omega(1/r)$, $\sum_i M_i(t)=1-O(\exp(-tr))$.
\end{lemma}
\begin{proof}
Follows immediately from 
$\sum_i M_i(t+1) = (1-r)\sum_i M_i(t)  + r$.
\comment{This recurrence gives,  
$\sum_i M_i(t) = (1-r)^{t} \sum_i M_i(0) + r \sum_{j=0}^t (1-r)^j +(1-r)^{t}( \sum_i M_i(0)  -1) $. Since $M_i(0)=0$, $\sum_i M_i(t)\leq 1$. 
Observe also that after t = $\Omega(1/r)$ steps this becomes $1+ O(exp(-tr))$}
\end{proof}

\begin{proof}(\textbf{Theorem~\ref{thm:gap1}})
To see that the solution to the given system is unique, note that $f_i = (\frac{v_i -u}{\alpha})^{+}$ (where $x^{+}$ denotes $max(x,0)$, and so
$\sum_i  (\frac{v_i -u}{\alpha})^{+} = 1$. This must have a unique solution as $\sum_i (\frac{v_i -u}{\alpha})^{+}$ is decreasing function of $u$ and strictly decreasing as long as the sum is positive.
Let $u$ denote the solution to the above system. 

We now show $\max_i u_i(t)\geq u$ for any $t$.  This is done by
contradiction. Suppose that for all $i$ $u_i(t)<u$.  We have that
$\sum_i(\frac{v_i-u}{\alpha_i})^{+}<
\sum_i \frac{v_i-u_i(t)}{\alpha_i}$. But $\sum_i \frac{v_i-u_i(t)}{\alpha_i} = \sum_i M_i(t)\leq 1$. We have that $\sum_i(\frac{v_i-u}{\alpha_i})^{+}<1$, a
contradiction. 


Let $S_g$ denote the set of all the items ever picked by the greedy
algorithm. Let $T$ be the time by which each item in $S_g$ has been
used at least once. By Lemma~\ref{lem:mem}, after some steps $\sum_i
M_i(t)$ converges to arbitrarily close to $1$. Lets assume for
simplicity of argument that it is exactly $1$ with sufficiently large
$T$. To show the upper-bound on $\max_i u_i(t)$, we show that for
$t\geq T$ and any $i\in S_g$, $\max_j u_j(t)-u_i(t)=O(\alpha r\log
n)$.

Denote by $x(t)$ the item that has the maximum utility at time $t$. 
It suffices to show that $u_{x(t)}(t)\leq u_i(t)+O(\alpha r \log n)$.
We recursively compute a decreasing sequence of $t_j$ as follows. Let
$t_1 = t$. For $j>1$, suppose we have computed $t_{j-1}$. Let $S_{j-1}
=
\{x(t_1),x(t_2),\cdots,x(t_{j-1})\}$. Now let
$t_j=\max_{t'<t_{j-1}, x(t')\notin S_{j-1}} t'$. We stop when there is
$k$ such that $x(t_k)=i$.  Since $t>T$, the process is guaranteed
to stop.  By the above construction, we know only items in
$S_{j-1}$ are picked by the greedy algorithm in the interval
$[t_{j}+1, t_1]$.  For any $S\subseteq \{1,\cdots, n\}$, let
$A(S,t)=\sum_{\ell\in S}\frac{u_\ell(t)}{\alpha_\ell}$, and $B(S)=
\sum_{\ell\in S}\frac{1}{\alpha_\ell}$.  We will show that for $1<j\leq k$.
\begin{equation}\label{eq:1}
A(S_{j-1},t_{j-1})\leq \frac{B(S_{j-1})}{B(S_j)}A(S_j, t_j)+r\,.
\end{equation}

First observe that
\begin{equation}\label{eq:2}
A(S,t)= \sum_{\ell\in S}\frac{u_\ell(t)}{\alpha_\ell}
=\sum_{\ell\in S}\frac{V_\ell -\alpha_\ell M_\ell(t)}{\alpha_\ell}
=\sum_{\ell\in S}\frac{V_\ell}{\alpha_\ell} -\sum_{\ell\in S} M_\ell(t)\,.
\end{equation}

(\ref{eq:1}) follows from the following claims.

\paragraph{Claim 1.} $A(S_{j-1},t_{j-1})\leq A(S_{j-1},t_j+1)$. 
\begin{proof}
Since any item picked by the greedy algorithm in $[t_j+1,t_{j-1}]$ is
in $S_{j-1}$, we have that for $t'\in [t_j+1,t_{j-1})$, $\sum_{\ell\in S_{j-1}}M_{\ell}(t'+1) = (1-r)\sum_{\ell\in S_{j-1}}M_{\ell}(t')+r
\geq \sum_{\ell\in S_{j-1}}M_{\ell}(t')$. The last inequality is by $\sum_{\ell} M_{\ell}(t')\leq 1$.  Therefore 
$\sum_{\ell\in S_{j-1}}M_{\ell}(t_{j-1})\geq
\sum_{\ell\in S_{j-1}}M_{\ell}(t_{j}+1)$. 
By (\ref{eq:2}), we have $A(S_{j-1},t_{j-1})\leq A(S_{j-1},t_j+1)$. 
\end{proof}

\paragraph{Claim 2.} $A(S_{j-1},t_j+1)\leq A(S_j, t_j)+r$. 
\begin{proof}
Since $t_j\notin S_{j-1}$ is the item picked by the greedy algorithm
at $t_j$, $\sum_{\ell\in S_{j-1}}M_{\ell}(t_j+1) = (1-r)\sum_{\ell\in S_{j-1}}M_{\ell}(t_j)$. Thus
$\sum_{\ell\in S_{j-1}}M_{\ell}(t_j+1)-\sum_{\ell\in S_{j-1}}M_{\ell}(t_j)
= r \sum_{\ell\in S_{j-1}}M_{\ell}(t_j) \leq r$. Again by (\ref{eq:2}), we have
 $A(S_{j-1},t_j+1)\leq A(S_j, t_j)+r$. 
\end{proof}

\paragraph{Claim 3.} $A(S_{j-1},t_j)\leq \frac{B(S_{j-1})}{B(S_j)}A(S_j, t_j)$.\begin{proof}
Immediately follows from $u_{t_j}(t_j)\geq u_{\ell}(t_j)$ for $\ell\in S_{j-1}$. 
\end{proof}
\medskip

Repeating (\ref{eq:1}), we have that
\begin{eqnarray*}
&&A(S_{j-1},t_{j-1})\\
&\leq& \frac{B(S_{j-1})}{B(S_j)}A(S_j, t_j)+r\leq \frac{B(S_{j-1})}{B(S_j)}\left(\frac{B(S_{j})}{B(S_{j+1})}A(S_{j+1}, t_{j+1})+r\right)+r\\
&=& \frac{B(S_{j-1})}{B(S_{j+1})}A(S_{j+1}, t_{j+1})+r\cdot\frac{B(S_{j-1})}{B(S_j)}+r \cdots \leq \frac{B(S_{j-1})}{B(S_k)}A(S_k, t_k)+r\cdot \sum_{\ell={j-1}}^{k-1} \frac{B(S_{j-1})}{B(S_\ell)}\,.
\end{eqnarray*}

Hence, we have that 

\[u_{x(t_1)}(t_1) = \alpha_1 A(S_1,t_1)\leq\alpha_1\left(\frac{B(S_1)}{B(S_k)}A(S_k, t_k)+r\cdot\sum_{\ell=1}^{k-1} \frac{B(S_1)}{B(S_\ell)}\right)=\frac{1}{B(S_k)}A(S_k, t_k)+r\cdot\sum_{\ell=1}^{k-1} \frac{1}{B(S_\ell)}\,.
\]

Since $i = x(t_k)$, for any $i'$, $u_{i'}(t_k)\leq u_i(t_k)$. 
Therefore  $A(S_k,t_k)=\sum_{j\in S_k}\frac{u_j(t_k)}{\alpha_j}
\leq u_i(t_k)\sum_{j\in S_k}\frac{1}{\alpha_j}=u_i(t_k)B(S_k)$.
By that $\alpha = \max_i \alpha_i$, we have 
$B(S_\ell) \geq \ell/\alpha$.  Hence

\[u_{x(t_1)}(t_1) \leq\frac{1}{B(S_k)}A(S_k, t_k)+r\cdot\sum_{\ell=1}^{k-1} \frac{1}{B(S_\ell)}\leq u_i(t_k)+\alpha r \sum_{\ell=1}^{k-1} 1/\ell = u_i(t_k)+ O(\alpha r \log n)\,.\]

\comment{
\begin{eqnarray*}
u_{x(t_1)}(t_1) &\leq &\frac{1}{B(S_k)}A(S_k, t_k)+r\cdot\sum_{\ell=1}^{k-1} \frac{1}{B(S_\ell)}\\
&\leq&u_i(t_k)+\alpha r \sum_{\ell=1}^{k-1} 1/\ell = u_i(t_k)+ O(\alpha r \log n)\,.
\end{eqnarray*}}

Since item $i$ is not used during the interval of $[t_k+1,t_1]$, we have 
$u_i(t_k+1)\leq u_i(t_1)$, and hence $u_i(t_k)\leq u_i(t_k+1)+\alpha_i r \leq u_i(t_1)+\alpha_i r$. Therefore we have that,
$\max_j u_j(t_1) = u_{x(1)}(t_1)\leq u_i(t_1)+ O(\alpha r \log n)$.

On the other hand, we know that there exists $i\in S_g$ such that $u_i(t)\leq
u$ because otherwise it would be the case that
$\sum_i(\frac{v_i-u}{\alpha_i})^+>\sum_i\frac{v_i-u_i(t)}{\alpha_i}=\sum_i
M_i(t)\approx 1$, a contradiction.  Hence $\max_j u_j(t)=u+O(\alpha r
\log n)$.
\end{proof}

\subsection{NP-hardness of item selection}

A selection $Y$ is periodic with period $T$, if for any $t$,
$y(t+T)=y(t)$, where $y(t)$ is the item chosen at time $t$.  Clearly,
in a periodic selection, the utility of the item chosen at time $t$ is
the same as the one chosen at time $t+T$.  For utility maximization,
it suffices to consider those items chosen in $[0,T)$.  Let
$U(Y)=\sum_{t=0}^{T-1} u_{y(t)}(t)$ denote the total utility of $Y$ in
$[0,T)$.

It is NP-hard to decide, given $T$, and $U^\ast$, and $n$ items,
whether there exist a assignment $Y$ with period $T$ such that
$U(Y)\geq U^\ast$.  The reduction is from the Regular Assignment
Problem~\cite{barnoy-02} and is detailed in the appendix.

\comment{
Consider the case when there is only one item. Given $T$, let $\Y_k$
be the set of all the selections which have period $T$ and choose the
item exactly $k$ times during $[0,T)$.  We claim that for any
$Y\in\Y_k$, $U(Y)\leq v-\alpha\frac{(1-r)^{T/k}}{1-(1-r)^{T/k}}$, and the equality
holds only when $Y$ is a regular assignment, i.e. when $k|T$ and any
two consecutive appearances are $T/k$ apart.

Consider $k$ appearances of the item in the real interval
$[0,T)$. Suppose that they appear at the time $t_0, \cdots, t_{k-1}$,
respectively.  Let $x_i = t_{i+1}-t_i$ for $0\leq i <k-1$ and $x_{k-1}
= t_0+T-t_{k-1}$.  For $0\leq i,j<T$, denote by $S_{ij}$ the set of
numbers from $i$ to $j$ inclusive, as considered on a cycle with
length $T$, i.e. when $i\leq j$, $S_{ij} =
\{i,i+1,\cdots, j\}$ and when $i>j$, $S_{ij} = \{i,i+1,\cdots, T-1\}
\cup
\{0,1,\cdots, j\}$.  Denote by $X_{i,j} = \sum_{\ell\in S_{ij}} x_\ell$. 


Because the selections are periodic, the memory at time $t_i$ is:
\[M_i = \frac{1}{1-(1-r)^T}\sum_{j=0}^{k-1} (1-r)^{X_{i,(i+j)\mod k}}\,.\]

Let $M = (1-(1-r)^T)\sum_{i=0}^{k-1} M_i$. Rearranging the terms in
the sum, we have that
\[M=\sum_{\ell=0}^{k-1}\sum_{i=0}^{k-1} (1-r)^{X_{i,(i+\ell)\mod T}}\,.\]

For any $\ell$, $\sum_{i=0}^{k-1} X_{i,(i+\ell)\mod T} = (\ell+1)T$
since each $x_i$ appears exactly $\ell+1$ times in the sum and
$\sum_{i} x_i = T$.  The sum $\sum_{i=0}^{k-1}
(1-r)^{X_{i,(i+\ell)\mod T}}$ is minimized when $X_{i,(i+\ell)\mod T}$
are all equal for $0\leq i<k$.  Therefore, $M$ is minimized when the
$k$ items are evenly spaced, and the minimum value is
$\sum_{i=0}^{k-1} (1-r)^{i+1} = (1-r)^{T/k}\frac{1-(1-r)^T}{1-(1-r)^{T/k}}$.
Since $\sum_i u_i = k v_i - \alpha \sum M_i = k v_i -\alpha
\frac{1}{1-(1-r)^T} M $, we have proven the claim.}




\subsection{Optimality of double-greedy algorithm}

Using the exactly same argument in the proofs of
Theorem~\ref{thm:gap1}, we have that

\begin{lemma}\label{lem:gap2}
There exists a time $T$ such that for any $t\geq T$, 
$\mu  \leq \max_i w_i(t)\leq \mu + O(\alpha \log n r)$ where $\mu$ 
is the unique solution to
the following system:

For all items with $f_i > 0$,  the quantity $v_i - 2 f_i \alpha_i = \mu$;
if $f_i = 0$ then $v_i < \mu$; and
$\sum f_i =1$.
\end{lemma}

By using the above lemma, we can now prove Theorem~\ref{thm:double-greedy}.
\begin{proof}(\textbf{Theorem~\ref{thm:double-greedy}})
For $0< f\leq 1$, write $\Delta(f)
=r\cdot\frac{(1-r)^{1/f}}{1-(1-r)^{1/f}}$.  

Let $U^\ast$ be the optimal value of the following program.
\begin{equation}\label{eq:0}
\max U = \sum_i f_i(v_i - \alpha_i f_i) \quad \mbox{s.t.}\quad \sum_i f_i\leq 1 \quad \mbox{and $f_i\geq 0$.}
\end{equation}

Let $OPT$ denote the optimal average utility. We have that $OPT\leq
U^\ast+\alpha r$.  This is by observing that for any $0<f<1$, placing
an item $1/f$ apart gives an upper bound on the utility of consuming
the item with frequence $f$.  The bound is $v-\alpha
\Delta(f) \leq v-\alpha(r-f)$ by observing that
 $\Delta(f)>r-f$.

The objective of (\ref{eq:0}) is maximized when there exists $\lambda$
such that $\frac{\partial U}{\partial f_i}=\lambda$ for $f_i>0$ and
$\frac{\partial U}{\partial f_i}<\lambda$ for $f_i=0$, and $\sum_i f_i
= 1$.  Since $\frac{\partial U}{\partial f_i} = v_i - 2\alpha_i f_i$,
$\lambda$ is exactly the same as $\mu$ in the statement of
Lemma~\ref{lem:gap2}. This explains the intuition of the double greedy
heuristics --- it tries to equalize the marginal utility gain of each
item.

Denote the optimal solution by
$f_i^\ast$. Then for $f_i^\ast>0$, $v_i - 2\alpha_i f_i^\ast = \mu$. Hence,
\[U^\ast = \sum_i
f_i^\ast(v_i-\alpha_i f_i^\ast) = \sum_i f_i^\ast
(\mu+\alpha_i f_i^\ast ) = \mu+\sum_i \alpha_i {f_i^\ast}^2\,.\]

Let $k_i$ denote the number of times item $i$ is used in $[0,T]$ by
the double-greedy algorithm, and $f_i = k_i/T$.  Let $\overline{M}_i$
denote the average memory on $i$ at the times when $i$ is picked.
Then we have that

\begin{eqnarray}
\overline{U}&= &\sum_{t=0}^T u_{x(t)}(t)/T=\sum_i \sum_{x(t)=i} u_i(t)/T=\sum_i \sum_{x(t)=i} (w_i(t)+\alpha_i M_i(t))/T\nonumber\\
&\geq&\sum_i \sum_{x(t)=i} (\mu+\alpha_i M_i(t))/T \quad\mbox{(by Lemma~\ref{lem:gap2}, $w_i(t)\geq \mu$)}\nonumber\\
&\geq&\mu + \sum_i \alpha_i f_i \overline{M}_i\,.\label{eq:3}
\end{eqnarray}

Write $\delta = \alpha r \log n$.  By Lemma~\ref{lem:gap2},
$w_i(t)=\mu + O(\delta)$ for each $i,t$.  We will show that

\paragraph{Claim 1. $\alpha_i f_i = \alpha_i f_i^\ast - O(\delta)$.}
Observe that for any item $i$ which is picked $k_i$ times in $[0,T]$,
$\min_{0\leq t\leq T} M_i(t)\leq \Delta(k_i/T)\leq k_i/T=f_i$.  Hence, $\max_t w_i(t)\geq v_i -
2\alpha_iM_i(t) \geq v_i - 2\alpha_i f_i $. On the other hand, $w_i(t)
= \mu + O(\delta)$.  
We have $v_i - 2\alpha_i f_i = \mu+O(\delta)$. But $\mu = v_i -
2\alpha_i f_i^\ast$. Therefore $\alpha_i f_i \geq \alpha_i f_i^\ast - O(\delta)$. 

\paragraph{Claim 2. $\alpha_i \overline{M}_i = \alpha_i f_i^\ast -O(\delta)$.}
Since $v_i - 2\overline{M}_i \leq \mu + \delta$, we obtain the bound by the same argument.

Now, plugging both claims into (\ref{eq:3}), we have that
\[\overline{U}\geq \mu + \sum_i \alpha_i (f_i^\ast -\frac{O(\delta)}{\alpha_i})^2 \geq \mu + \sum_i \alpha_i {f_i^\ast}^2 - O(\delta)
= U^\ast - O(\delta)
 = OPT-O(\delta)\,.\]

This last equality follows from $U^\ast = OPT - \alpha r$. 
This completes the proof. 
\end{proof}

\subsection{Social Choice is equivalent to individual choice}

Let $\ones$ denote the vector with all coordinates set to $1$ and $\valpha_i$ denote the vector of boredom coefficients $\alpha_{ij}$.

\paragraph{Observation.}
For any diagonolizable matrix $A$ with largest eigenvalue $1$ and the second largest eigenvalue is at most $1-\eps$, there is a vector $c$ so that.
$\ones' A^t x - c' x \le  (1-\eps)^t \sqrt n O(|x|_2)$. The $O$ notation hides factors that depends on $A$. For a real, symmetric matrix the constant is $1$.
\begin{proof}
We will sketch the proof for real symmetric matrices. The same idea holds for non-symmetric matrices.
If $p_1, \ldots, p_n$ denote the eigenvectors of $A$ and $1=\lambda_1, \ldots, \lambda_n$ denote the eigenvalues then
$A^t x = \sum_j \lambda^t_j p_i v'_i x = p_1 v'_1 x +  \sum_{j>1} {\lambda^t}_j p'_i p_i x$.
Now,|$\sum_{j>1} \lambda^t_j p'_i p_i x|_2 \le (1-\eps)^t |x|_2$.
So $|\ones'(A^t x - p_1 p'_1 x)| \le  |\ones|_2 (1-\eps)^t |x|_2 = \sqrt n (1-\eps)^t |x|_2$
Setting $c = \ones' v_1 v'_1$ completes the proof.
\end{proof}

We will now prove theorem~\ref{thm:socialchoice}
\begin{proof}(\textbf{Theorem~\ref{thm:socialchoice}})
Let $\Delta \b(t)$ denote $\b(t) -\b(t-1)$.
Now $\u_i (t) =  A \u_i(t-1) + \Delta \b(t)$. This gives, $\u_i(t) =  A^t \v_i  + \sum_{j=0}^{t-1} A^j \Delta \b (t) $.
Note that $W_i(t)$ = $\ones' \u_i(t) =\ones'  A^t \v  + \sum_{j=0}^{t-1} \ones' A^j \Delta\ b (t-j) $

Note that $\Delta b_{ij} (t) = \alpha_{ij} ((1-r) M_{ij}(t)  + r I_i (t) - M_{ij} (t)) =  \alpha_{ij} r( x_i (t) - M_{ij} (t))$.
So $|\Delta b_{ij} (t)|_2 \le r |\valpha_{i}|_2$.

%Let $l = \Theta((1/\eps)log(1/r))$. For this value of $l$, $(1-\eps)^l \le r$.
%We will separtely bound in the range $i \le l$ and $i \ge l$.

Now  $|\ones' A^t \v_i - c' \v_i| \le (1-\eps)^t \sqrt n O(|\v_i|_2)$. For $t> (1/\eps)\Omega( \log( nr|\v_i|_2) $, this is at most $r$.
Also  $|\ones A^j \Delta \b_i (t-j) - c' \Delta \b_i (t-j)| \le  (1-\eps)^j  \sqrt n O( |\Delta  \b_i (t-j)|_2) \le (1-\eps)^j  \sqrt n rO( | \valpha_i|_2) $.
So,  $|\sum_j \ones A^j \Delta \b_i (t-j) - \sum_j c' \Delta \b_i (t-j)| \le (r/\eps) \sqrt n O(|\valpha_i|_2)$.
So,  $|\sum_j \ones A^j \Delta \b_i(t-j) - c'\ b_i (t)| \le (r/\eps)  \sqrt n O(|\valpha_i|_2)$.
Therefore $|W_i (t) - (c'\v_i - c' \b_i(t))| \le (r/\eps) O(\sqrt n  |\valpha_i|_2)$. Dividing by $n$ completes the proof.
\end{proof}





